Learning-Based Adaptive User Selection in Millimeter Wave Hybrid Beamforming Systems

We consider a multi-user hybrid beamforming system, where the multiplexing gain is limited by the small number of RF chains employed at the base station (BS). To allow greater freedom for maximizing the multiplexing gain, it is better if the BS selects and serves some of the users at each scheduling instant, rather than serving all the users all the time. We adopt a two-timescale protocol that takes into account the mmWave characteristics, where at the long timescale an analog beam is chosen for each user, and at the short timescale users are selected for transmission based on the chosen analog beams. The goal of the user selection is to maximize the traditional Proportional Fair (PF) metric. However, this maximization is non-trivial due to interference between the analog beams for selected users. We first define a greedy algorithm and a "top-k" algorithm, and then propose a machine learning (ML)-based user selection algorithm to provide an efficient trade-off between the PF performance and the computation time. Throughout simulations, we analyze the performance of the ML-based algorithms under various metrics, and show that it gives an efficient trade-off in performance as compared to counterparts.

==> extra.tex <==
\nextbf{EXTRA WRITE UP}

\textbf{User Selection \rev{(Main focus)}}

User selection should be conducted within a short time scale as compared to the analog beamforming. Although the current  VIF-based user selection algorithm (refer to the user selection document) works, it needs quite a long computation time to obtain the result of the selected users.
We note that the user selection is conducted at the BS.
Since we are in need of a \textit{fast inference} for user selection, we will construct the neural network (NN) to replace the current user selection algorithm.
Also, we want to minimize the size of inputs to have \textit{a low feedback overhead} caused by gathering information  from the users.
We first define the potential inputs and outputs for the NN.

\textbf{Inputs}


\textbf{Outputs}

For the output variables, we introduce a binary output vector as ${\bf a}(t) = [{a}_1(t), ..., {a}_I(t)]^T$ where ${a}_i(t) \in \{0,1\}$ represents whether the BS selects user $i$ to serve at time $t$. Then, the size of output is $I$.
As the output of the training data, we can use the outputs from the VIF-based user selection algorithm.

\textbf{Baseline 1. Exhaustive search}
1. Computational complexity
2. Feedback overhead (For a start, we assume all information is fed back, so we don't consider the feedback overhead)

\textbf{Baseline 2. Selection based on the $M$ highest beam gains}

\textbf{Baseline 3. The VIF-based algorithm}

\textbf{Digital Beamforming}
Once the users are selected, the BS can construct the RF precoders as
\begin{equation}
    {\bf F}^\star_{\rm RF}(t) = [{\bf f}^\star_{{\rm RF},i_1(t)}(t), ..., {\bf f}^\star_{{\rm RF},i_M(t)}(t)].
\end{equation}
Also,  user $i$, $i \in \mathcal{M}(t)$, has the RF combiner as ${\bf u}^\star_{i}(t)$. 
Note that user $i$ measures 
the effective channel given by
\begin{align}
    {\bf h}_i(t) = ({\bf u}^{\star H}_{i}(t) {\bf H}_i(t) {\bf F}^\star_{\rm RF}(t))^H \in \mathbb{C}^{ M \times 1 }.
\end{align}
The BS receives a quantized version of the effective channel, $\hat {\bf h}_i(t)$, via feedback from user $i$, $i \in \mathcal{M}(t)$.
The BS then constructs
\begin{align}
    \hat {\bf H}(t) = [\hat {\bf h}_{i_1(t)}(t), ..., \hat {\bf h}_{i_M(t)}(t)]^H \in \mathbb{C}^{ M \times M}.
\end{align}
We adopt a zero-forcing (ZF) beamforming to design the digital precoder, which requires ${\bf F}_{\rm BB}(t)$ to satisfy
$\hat {\bf H}(t) {\bf F}_{\rm BB}(t) = {\bf I}$.
Then, the BS constructs the digital precoder by taking the right pseudo inverse of $\hat {\bf H}(t)$, given by
\begin{align}
    {\bf F}^\star_{\rm BB}(t) & =  (\hat {\bf H}(t))^\dagger 
    \\
    & = \hat {\bf H}^H(t) (\hat {\bf H}(t)\hat {\bf H}^H(t))^{-1}
\end{align}
We then normalize each column of ${\bf F}^\star_{\rm BB}(t) = [{\bf f}^\star_{{\rm BB},i_1(t)}(t), ..., {\bf f}^\star_{{\rm BB},i_M(t)}(t)]$ to satisfy the total transmission power constraint. In this work, we consider an equal power allocation for the $M$ data streams, i.e., $\| {\bf F}^\star_{\rm RF}(t) {\bf f}^\star_{{\rm BB},i}(t) \|^2 = \frac{P}{M}$, $i \in \mathcal{M}(t)$.
To this end, we normalize each column as
\begin{align}
    {\bf f}^\star_{{\rm BB},i}(t) \leftarrow  \sqrt{\frac{P}{M}} \frac{{\bf f}^\star_{{\rm BB},i}(t)} {\| {\bf F}^\star_{\rm RF}(t) {\bf f}^\star_{{\rm BB},i}(t) \|_2}, \quad i \in \mathcal{M}(t).
\end{align}
\rev{(We may want a non-equal power allocation to maximize the weighted sum-rate. Generally, we may want a different beamforming method rather than ZF for weighted sum-rate maximization, e.g., WMMSE method~\cite{shi2011iteratively}.)}


Inputs could be $\{{\bf h}^H_i {\bf f}_p\}_{i,p}$ and $\{w_i\}_i$.
Outputs could be ${\bf a} = [a_1, ..., a_I] \subset \{ 0,1 \}^{I}$, from which we can construct $\mathcal{M} = \{ i: \; a_i=1, \; i =1,...,I \}$.

$\\$
\q{Questions.}

How to determine ${\bf F}_{\rm BB}$? Do we determine it with ZF after the NN inference? 

Knowing $\{{\bf h}^H_i {\bf f}_p\}_{i,p}$ may be enough to solve it analytically? But it may be slow. Need to make sure why we need NN ... b/c we need a fast inference? Or, b/c we have limited measurements?

Why is the greedy algorithm  slow? b/c large $I$ is considered? Not done per approx. msec?

In simulations, the channels are varying in a long time scale or a short time scale ? Probably, long.

--Understand Greedy+VIF Alg?  Try NN? 

--Could develop another greedy alg, Greedy+WMMSE alg. Add users one by one by calculating WSR based on WMMSE. May need $I + (I-1) + ... + (I-M+1)$ combinations to calculate.

